TRECVID 2020: A comprehensive campaign for evaluating video retrieval tasks across multiple application domains

The TREC Video Retrieval Evaluation (TRECVID) is a TREC-style video analysis and retrieval evaluation with the goal of promoting progress in research and development of content-based exploitation and retrieval of information from digital video via open, metrics-based evaluation. Over the last twenty years this effort has yielded a better understanding of how systems can effectively accomplish such processing and how one can reliably benchmark their performance. TRECVID has been funded by NIST (National Institute of Standards and Technology) and other US government agencies. In addition, many organizations and individuals worldwide contribute significant time and effort. TRECVID 2020 represented a continuation of four tasks and the addition of two new tasks. In total, 29 teams from various research organizations worldwide completed one or more of the following six tasks: 1. Ad-hoc Video Search (AVS), 2. Instance Search (INS), 3. Disaster Scene Description and Indexing (DSDI), 4. Video to Text Description (VTT), 5. Activities in Extended Video (ActEV), 6. Video Summarization (VSUM). This paper is an introduction to the evaluation framework, tasks, data, and measures used in the evaluation campaign.

==> smkbp.tex <==
The 2018 Streaming Multimedia Knowledge Base Population (SM-KBP) evaluation is a new pilot task jointly run by the Text Analysis Conference. 
The task tries to address the need for technologies to analyze and extract knowledge from multimedia to support answering questions and queries to respond to the situations such as natural disasters or international conflicts. In such situations, analysts and the public are often confronted with a variety of information coming through multiple media sources.  The streaming multimedia extraction task asks systems to extract knowledge elements (KEs) from heterogeneous multimedia sources such as text documents, images, videos, audio, social media sites, etc. Although the big picture of the task is to use those knowledge elements to populate a knowledge base and later on to answer questions, TRECVID participants only had the opportunity to work on the first stage (denoted here as "TA1") of the task and mainly to analyze the video data stream to extract detectable knowledge elements based on a provided ontology.

\subsection{Task Definition}
TA1 systems are expected to process one document at a time (single document processing) and produce a set of KEs for each input document from the document stream. This is referred to as a document-level knowledge graph. 
A knowledge graph (KG) represents all knowledge, whether it comes from the document stream or some shared background knowledge, or via insertion of knowledge by a human user. A KE is a node or edge in a knowledge graph. Knowledge element types are defined in the ontology. A node in the knowledge graph represents an Entity/Filler, Event, or Relation, and an edge links an event or relation to one of its arguments.
A KE represents a single entity, a single event or a single relation. The KE maintains a cluster (or a node) of all mentions from within the document of the same entity, and a cluster (or node) of one or more mentions of each event or relation. An entity cluster should group together entity mentions that are referring to the same real-world entity. The same is true with events and relation clusters, though the definition of equality (coreference) may be fuzzier than for entities.

A document may contain document elements in multiple modalities and multiple languages; therefore, cross-lingual and cross-modal entity and event coreference are required. Conceptually, TA1 system must process each document in the order given in the document stream and must freeze all output for a document before starting to process the next document in the stream; however, because TA1 is stateless across documents (i.e., TA1 must process each document independently), in practice for the pilot evaluation, TA1 may choose to parallelize processing of documents for efficiency. NIST will evaluate output for only selected documents in the data stream, via pooling and assessment.

\subsection{SM-KBP Data}
For the 2018 pilot, the conflict scenario chosen was the Russian/Ukrainian conflict (2014-2015). A training corpus of 10\,000 documents were released by LDC and included at least between 1200 and 1500 topic-relevant and/or scenario relevant documents. The training corpus included data addressing a set of 6 training topics as follows:
\begin{itemize}
    \item{Crash of Malaysian Air Flight MH17 (July 17, 2014)}
    \item{Flight of Deposed Ukrainian President Viktor Yanukovych (February 2014)}
    \item{Who Started the Shooting at Maidan? (February 2014)}
    \item{Ukrainian War Ceasefire Violations in Battle of Debaltseve (January-February 2015)}
    \item{Humanitarian Crisis in Eastern Ukraine (July-August 2014)}
    \item{Donetsk and Luhansk Referendum, aka Donbas Status Referendum (May 2014)}
\end{itemize}

One evaluation topic and about 10\,000 documents were released as testing data:

\begin{itemize}
    \item{Siege of Sloviansk and Battle of Kramatorsk (April-July 2014)}
\end{itemize}
The distributed corpus included different modalities such as videos, images, html web pages, tweets, audio and pdf files. For all the video data, NIST released a shot boundary reference table that maps each whole video to several shot segments to be used by systems in their run submissions.

Task participants also received an ontology of entities, events, event arguments, relations, and SEC (sentiment, emotion, and cognitive state), defining the KEs that are in scope for the evaluation tasks.

\subsection{Evaluation Queries}
NIST distributed a set of evaluation queries to TA1 participants to apply to their output knowledge graphs. The queries in general tested a system for its effectiveness in determining the presence of a knowledge element or knowledge graph in the document collection, where a document may contain multiple document elements, and each document element can be text, video, image, or audio. Broadly, queries may be one of three types:

\begin{itemize}
    \item {Class level queries:} The query will provide a type from the ontology, and the teams will be asked to return all mentions of the class corresponding to the given type (e.g Person, Organization, Geopolitical Entity, Facility, Location, Weapon, Vehicle).
    \item{Instance level queries} (a.k.a. “zero-hop queries”): The query will provide a mention of an entity or filler from the ontology, and the teams will be asked to return all mentions of that particular entity/filler. For e.g., the query may ask for all mentions of “Jack Bauer” referred to in document 32 at offset 100-110.
    \item{Graph queries:} The query will be composed of a combination of ontology types and their instances and ask for a connected graph with at least one edge.
\end{itemize}

Teams were provided queries in two formats, which are intended to be semantically equivalent:
\begin{itemize}
    \item {Simplified:} Simplified query in an XML format that teams may apply to their KBs using any automatic technique that they choose. These simplified queries will be expressed in the domain ontology and are intended to be human-readable but will not be executable using standard tools.
    \item{Executable:} Executable SPARQL query that teams should apply using a dockerized tool provided by NIST; subsequently, NIST would use the same tool to apply executable queries in a uniform way to all KBs from all teams.
\end{itemize}


\subsection{Measures}
Teams were asked to submit the whole knowledge base (KB) in addition to xml response files to the evaluation queries. All responses required a justification grounded in the documents (e.g text span, video shot, image ID, etc). All mentions returned in response to a class-based query requesting a particular type (e.g., “Location”) or to a zero-hop query requesting mentions of a particular entity/filler (e.g., “Vladimir Putin”) in a “core” subset of the evaluation documents, were assessed by LDC for correctness. Graphs returned in response to graph queries are broken into assessment triples (subject justification, object justification, predicate justification) for assessment by LDC. Evaluation scores are based on F1 of Precision and Recall. For more details on the guidelines and evaluation measures and procedures please refer to the detailed evaluation plan of the task(s) provided by TAC \footnote{https://tac.nist.gov/2018/SM-KBP/guidelines/SM-KBP\_2018\_Evaluation\_Plan\_V0.8.pdf}

%\subsection{Results}


